Channel Simulation and Distributed Compression with Ensemble Rejection Sampling

We study channel simulation and distributed matching, two fundamental problems with several applications to machine learning, using a recently introduced generalization of the standard rejection sampling (RS) algorithm known as Ensemble Rejection Sampling (ERS). For channel simulation, we propose a new coding scheme based on ERS that achieves a near-optimal coding rate. In this process, we demonstrate that standard RS can also achieve a near-optimal coding rate and generalize the result of Braverman and Garg (2014) to the continuous alphabet setting. Next, as our main contribution, we present a distributed matching lemma for ERS, which serves as the rejection sampling counterpart to the Poisson Matching Lemma (PML) introduced by Li and Anantharam (2021). Our result also generalizes a recent work on importance matching lemma (Phan et al, 2024) and, to our knowledge, is the first result on distributed matching in the family of rejection sampling schemes where the matching probability is close to PML. We demonstrate the practical significance of our approach over prior works by applying it to distributed compression. The effectiveness of our proposed scheme is validated through experiments involving synthetic Gaussian sources and distributed image compression using the MNIST dataset.

==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page limit. 

%Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
%\begin{itemize}
%    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
%\end{itemize}

%{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

%The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

%IMPORTANT, please:
%\begin{itemize}
%    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
%\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes we support every claim in the abstract with proof and experimental results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See the Conclusion Section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Every assumption is rigorously stated.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code will be included for reproducibility.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Code will be available upon acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See the Experiment Section. 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Every plot is averaged for 10 different random seeds.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: See the experiment section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We check and verify the paper follows the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper poses no such societal impacts due to its scope in compression and information theory.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper focuses on probabilistic methods and poses no such risk.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No assets involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No assets involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  This paper provides theoretical studies of channel simulation and does not involve related items.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This paper provides theoretical studies of channel simulation and does not involve related items.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No LLM usage was involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> gaussian_exp.tex <==
\begin{figure}[t]
\vspace{-15pt}
  \centering
  \begin{minipage}[b]{0.74\textwidth}
    \centering
    \includegraphics[width=01.0\textwidth]{Neurips2025/figures/merged_Gaussian.pdf}
    \vspace{-35pt}
  \end{minipage}
  \hspace{2pt}
  \begin{minipage}[b]{0.23\textwidth}
  \centering
  \raisebox{20pt}{ % adjust value as needed
    \small
    \begin{tabular}{|c|c|}
      \hline
      $N^* $ & Target $\mathrm{dB}$ \\
      \hline
      $0.48\mathrm{e}6$ &  $-21\mathrm{dB}$\\
      $0.55\mathrm{e}6$ &  $-21.5\mathrm{dB}$\\
      $0.95\mathrm{e}6$ &  $-22\mathrm{dB}$\\
      $1.05\mathrm{e}6$ &  $-22.5\mathrm{dB}$\\
      $1.14\mathrm{e}6$ & $-23 \mathrm{dB}$\\
      \hline
    \end{tabular}
    \normalsize
  }
\end{minipage}
\vspace{10pt}
  \caption{\textit{Left}: Comparison of RD performance between different matching results for the Gaussian setting when targeting $-23\mathrm{dB}$ distortion (\textbf{black dotted line}), with the average number of proposals $N^*\in \{1.1\mathrm{e}6,1.6\mathrm{e}6\}$. \textit{Right}: RD curves of different methods. Each group targets the same distortion levels and uses the same average number of proposals $N^*$ for ERS and IML, shown in the right table.}
  \label{fig:Gauss_exp}
  \vspace{-12pt}
\end{figure}

\begin{table}[h]
\centering
\scriptsize
\begin{tabular}{ll}
\toprule
\textbf{Distribution} & \textbf{Expression} \\
\midrule
\(Q_{Y'}(\cdot)\) & \(\mathcal{N}(0, \sigma^2_{Y'})\) \\
\(P_{Y'|X}(\cdot\,|\,x)\) & \(\mathcal{N}(x, \sigma^2_{Y'|X})\) \\
\(P_{Y'|X'}(\cdot\,|\,x')\) & \(\mathcal{N}\left(x' \frac{\sigma^2_X}{\sigma^2_{X'}}, \, \sigma^2_{Y'} - \frac{\sigma^4_X}{\sigma^2_{X'}}\right)\) \\
\bottomrule
\end{tabular}
\caption{Definitions of the relevant distributions.}
\label{tab:distributions}
\end{table}


==> old/ERS_Matching_old.tex <==
\subsection{Distributed Matching Probabilities}
\begin{figure*}[t]%
    \centering%
    \vspace{-25pt}
    \hspace{15mm}
        \includegraphics[width=0.95\linewidth]{Neurips2025/figures/Matching_Plot3.pdf}%
    \vspace{-6pt}
   \caption{(Best viewed in color)  We set $Q_Y{=}\mathcal{N}(0,100)$, $P^A_Y{=}\mathcal{N}(0.5, 0.7)$ and $P^B_Y{=}\mathcal{N}(-0.5,0.7)$. \textit{Left}: Matching probabilities versus the batch size \( N \). \textit{Middle}: Matching probabilities versus the average number of proposals where the \textbf{\textcolor{red}{red}} and \textbf{\textcolor{black}{black}} dotted lines correspond to the batch sizes \( \omega \) and \( 4\omega \) shown in the left figure. \textit{Right}: Sample quality of IS, measured by the estimated variance \( \hat{\sigma}^2 \).}
    \label{fig:match_compare}
     \vspace{-12pt}
\end{figure*}
\textbf{Matching Setup.} Intuitively, since both parties tend to accept the first batch for a large enough $N$ as $\Delta \xrightarrow[]{} 1.0$,  the matching probability of ERS approaches that of IML  and  PML. We discuss the matching setup where the encoder (party $A$)  send the accepted batch index $K_{1,A}$ to the decoder (party $B$), which is useful for practical purposes.  The case without batch communication is shown in Appendix \ref{no_batch_comm}.  Consider the conditional distributed matching scenario, which generalizes the one described in Section \ref{sec:rs_distributed_matching}: Let  $(X,Y,Z)$ be a triplet of random variables with a joint distribution $P_{X,Y,Z}(.)$  satisfying the bounding condition
$\max_{y}\left({P_{Y|X}(y|x)}{Q^{-1}_Y(y)}\right) \leq \omega,
$  
where $Q_Y(.)$ is the proposal distribution within $W$. The communication protocol works as follows.

%\textbf{Matching Setup. } We focus on the matching probability when the encoder (party \( A \)) communicates the selected batch index $K_{1,A}$ to the decoder (party \( B \)), which is useful for practical purposes. The case without batch communication is shown in Appendix \ref{no_batch_comm}. We consider the conditional distributed matching scenario, which generalizes the one described in Section \ref{sec:rs_distributed_matching}: Let  $(X,Y,Z)$ be a triplet of random variables with a joint distribution $P_{X,Y,Z}(.)$  satisfying the bounding condition
%$\max_{y}\left({P_{Y|X}(y|x)}{Q^{-1}_Y(y)}\right) \leq \omega,
%$  
%where $Q_Y(.)$ is the proposal distribution within $W$. The communication protocol works as follows.
\begin{itemize}
    \item Step 1: Given $X{=}x$ sampled independently of $W$, the encoder uses ERS and obtain the index $K_A$ with $Y_{K_A}{\sim }P^A_Y(.) {=}P_{Y|X}(.|x)$. It then sends the batch index $K_{1,A}$ to the decoder.
    \item Step 2: Given $X=x,Y_{K_A}=y$, we generate $Z\sim P_{Z|X,Y}(.|x,y)$ and note that the following Markov chain $Z-(X,Y)-W$ is satisfied by this reconstruction. In practice, $Z$ can be some correlated information or messages from the encoder.
    \item Step 3:  After obtaining $Z{=}z$ and the batch index $K_{1,A}$, the decoder use the Gumbel-IS to select the index $\Tilde{K}_B$ within batch $K_{1,A}$ with target distribution $P^B_Y(.){=}\Tilde{P}_{Y|Z}(.|z)$, i.e.:
    \begin{align}
        \Tilde{K}_B = \operatorname*{argmin}_{1\leq k \leq N} \frac{S_{i, k}}{\lambda_{i,k}}, \text{ where } \lambda_{i,k} = \frac{\Tilde{P}_{Y|Z}(Y_{ik}|z)/Q_Y(Y_{ik})}{\sum^N_{j=1}\Tilde{P}_{Y|Z}(Y_{ij}|z)/Q_Y(Y_{ij}))} \text{ and } i =K_{1,A}
    \end{align}
\end{itemize}
%Given $X=x$ sampled independently of $W$, the encoder use ERS to sample the index $K_A$ and the associate $Y_{K_A}$ following the distribution $P_{Y|X}(.|x)$. Given $X=x,Y_{K_A}=y$, let $Z\sim P_{Z|X,Y}(.|x,y)$ and note that the following Markov chain $Z-(X,Y)-W$ is satisfied by this reconstruction. In practice, $Z$ can be some correlated information or messages from the encoder. The decoder obtains $Z=z$ and use the ERS procedure on $W$ with target distribution $\Tilde{P}_{Y|Z}(.|z)$.

%In practice, the target distribution $P_{Y|X}(.|x)$ at the encoder can be predetermined to ensure that the ratio $\frac{P_{Y|X}(y|x)}{Q_Y(y)}$ remains bounded for all $y$. 

%Even when the ratio ${\Tilde{P}_{Y|Z}(y|z)}/{Q^{-1}_Y(y)}$ at the decoder side is unbounded,
Exact sampling schemes like ERS (and PML) rely on the bounding condition to terminate but this value in practice is difficult to establish for the ratio ${\Tilde{P}_{Y|Z}(y|z)}/{Q^{-1}_Y(y)}$ at the decoder, which is often estimated via neural networks. Thus, limiting the selection process to a specific batch ensures termination.  We have the following bound for the matching probability.

%To address this, the encoder can transmit the index of the selected batch to the decoder, ensuring that both parties complete the selection process. Despite introducing additional communication overhead, the cost is $O(1)$ for sufficiently large $N$ and negligible when jointly compressing multiple samples. 

\begin{proposition}\label{prop:match_ers_comm} Let $K_A, \Tilde{K}_B, P_{Y|X}(.|x)$ and $\Tilde{P}_{Y|Z}(.|z)$ defined as above. For $N\geq 2$, we have:
\begin{align}\label{prop:match_ers3}
    \Pr (Y_{K_A} = Y_{\Tilde{K}_B}|Y_{K_A} = y, X=x, Z=z) \geq \left({1 {+}\mu'_1(N) {+} \frac{P_{Y|X}(y|x)}{\Tilde{P}_{Y|Z}(y|z)} \left(1 + \mu'_2(N)\right)}\right)^{-1},
\end{align}
    where $\mu'_1(N)$ and $\mu'_2(N)$ are defined as in Appendix \ref{coefficient_match_lemma2} and we note that $\mu'_1(N), \mu'_2(N) \xrightarrow[]{} 0$ as $N\xrightarrow[]{} \infty$ with rate $N^{-1} $under mild assumptions on the distributions $P_{Y|X}(y|x)$ and $Q_Y(.)$. 
\end{proposition}
\begin{proof}
    See Appendix \ref{proof_match_ers_comm}.
\end{proof}
%\begin{remark}
%    Since the coefficients $\mu'_1(N),\mu'_2(N)\xrightarrow[]{}0.0$ with the rate $N^{-1}$, for any small $\epsilon$ one can choose $N$ large enough such that  $\mu'_1(N),\mu'_2(N) \leq \epsilon$. 
%\end{remark}

When $N=1$, the matching probability is $1.0$  and will gradually approach the matching probability of PML as $N\xrightarrow[]{}\infty$. Figure \ref{fig:match_compare} (left) validates and compares its matching probability with PML and IML. For the same average number of proposals, Figure \ref{fig:match_compare} (middle) demonstrates that ERS (with batch communication) achieves a consistently higher matching probability than IS, while maintaining an unbiased sample distribution. For completeness, Figure \ref{fig:match_compare} (right) shows the bias of IS, where we observe that the bias can remain even when the batch size is sufficiently large. We discuss the overhead for sending the batch index in Section \ref{wyner_ziv} on application to distributed compression.


%We consider the conditional case in Section \ref{no_batch_comm}. Let $K_{A}$ be as defined in Section \ref{no_batch_comm}, and let $\Tilde{K}_{B}$ denote the index selected by party $B$ within the batch chosen by party $A$, Proposition \ref{prop:match_ers_comm} provides a bound on the matching probability. In this case, we only require $\frac{P_{Y|X}(y|x)}{Q_Y(y)} \leq \omega$ for all $y$. 


%\begin{proposition}\label{prop:match_ers_comm} Let $K_A, \Tilde{K}_B$ and $P^A_Y, P^B_Y$ defined as above and $N\geq 2$, we have:
%\begin{align}\label{prop:match_ers3}
%    \Pr (Y_{K_A} = Y_{\Tilde{K}_B}|Y_{K_A} = y, X=x, Z=z) \geq \left({1 +\mu'_1(N) + \frac{P_{Y|X}(y|x)}{\Tilde{P}_{Y|Z}(y|z)} \left(1 + \mu'_2(N)\right)}\right)^{-1},
%\end{align}
%    where $\mu'_1(N)$ and $\mu'_2(N)$ are defined as in Appendix \ref{coefficient_match_lemma2} and we note that $\mu'_1(N), \mu'_2(N) \xrightarrow[]{} 0$ as $N\xrightarrow[]{} \infty$ under mild assumptions on the distributions $P_{Y|X}(y|x)$ and $Q_Y$. 
%\end{proposition}
%\begin{proof}
%    See Appendix \ref{proof_match_ers_comm}.
%\end{proof}






\subsubsection{Lossy Compression with Side Information} \label{wyner_ziv}
We consider an application of our matching results to the Wyner-Ziv distributed compression \cite{wyner1976rate}, where the decoder has access to the correlated side information $X'$ not available to the encoder. Specifically, let $X {=} x {\sim} P_X(\cdot)$ denote the input to the encoder, and let $X' \sim P_{X'|X}(\cdot|x)$ represent the above side information. Let $P_{Y|X}(.|x)$ be the encoder's target distribution, which together with $X'$ forms a joint distribution $P_{X,X',Y}$. For any integer $\mathcal{V}>0$, we define the common randomness $W$:
\begin{align}
     W &{=} \{ (B_1, U_1), (B_2, U_2), ...\}, \text{ where } U_i \sim  \mathcal{U}(0,1) \notag\\
    {B}_i&{=}\{(Y_{i1}, S_{i1}, V_{i1}),..., (Y_{iN}, S_{iN}, V_{iN})\}, \text{ where } Y_{ij} {\sim} Q_{Y}(.), S_{ij} {\sim} \mathrm{Exp}(1), V_{ij}{\sim} P_V (.) \notag,
\end{align}
where $P_{V}$ is $\text{Unif}[1{:}\mathcal{V}]$ and $\max_{y} P_{Y|X}(y|x)Q^{-1}_Y(y){\leq} \omega$. The encoder selects an index $K_A$ according to the target distribution $P^A_{Y|X,V}(y|x,v) = P_{Y|X}(y|x)P_V(v)$ and send the hash value $V_{K_A}$ and the batch index $K_{1,A}$  to the decoder. After receiving $Z{=}(X', V_{K_A})$ and $K_{1,A}$, the decoder sets its  target  $P^B_{Y|X',V}(y|x',v) = P_{Y|X'}(y|x')\mathbbm{I}_V(v)$, i.e. it removes all the index with different hashed value from $V_{K_A}$ and selects an index with IS. Applying Proposition \ref{match_lemma_cond} gives the following results:

\begin{proposition}
\label{prop_application}Fix any $\epsilon$,  for sufficiently large $N$, we have:
\begin{align}
&\Pr(Y_{K_A} \neq Y_{K_B}) \le   E_{X,Y,X'}\left[1- \left(1+ \epsilon + (1+\epsilon)\mathcal{V}^{-1} \textcolor{black}{2^{i(Y;X) - i(Y;X')}} \right)^{-1} \right]
\label{eq:err-bnd-main}
\end{align}
where \textcolor{black}{$i_{Y;X}(y;x) = \log \frac{P_{Y;X}(y;x)}{P_{Y}(y)}$} is the information  density. The coding cost is $\log(\mathcal{V}) + r$ where $r$ is the coding cost of sending the selected batch and $r\leq 4$ bits for $N \geq \omega'$ where $\omega' = \max_{x,y}P_{Y|X}(y|x)Q^{-1}_Y(y)$, i.e. when average batch acceptance probability $\Delta\geq 0.5$. 
\end{proposition}
\begin{proof}
    See Appendix \ref{proof_prop_application}
\end{proof}
\begin{remark}\label{remark_wyner}
With a sufficiently large batch size $N$, jointly compressing $n$ samples reduces the overhead upper-bound to $4/n$ per sample. Furthermore, this also lowers the error probability, given that $\log(V) \geq nI(Y;X|X')$ (see Appendix \ref{proof_prop_application}). Finally, in practice, we use the following formula for the number of samples required in IS \cite{chatterjee2018sample} as a starting point for choosing the batch size $N$, i.e. $N=2^{\mathbb{E}_X[D_{KL}(P_{Y|X}(.|x)||Q_Y(.)]+t}$ where $t\geq4$ often gives $\Delta \geq 0.5$, resulting in a small overhead $r$.
\end{remark}


%Unlike channel simulation, the decoder's received output is biased due to mismatched probabilities. However, obtaining an exact sample at the encoder is valuable for broadcasting messages to multiple clients, especially when some lack access to side information and require direct communication, as in standard channel communication. In addition, a feedback mechanism can be employed to rectify the error \cite{phan2024importance} and thus recover the unbiased samples. 

%\textbf{Practical Implementation. }
% Note that the joint distribution $P_{X,X'}$ represents the data distribution, which is unknown in practice. Thus one needs to rely on machine learning to estimate $P_{Y|X'}(y|x)$ but due to the non-convex nature of neural networks, it is not trivial to obtain the upperbound of $P_{Y|X'}(y|x)Q^{-1}_Y(y)$ to decide termination in PML.

%\begin{remark}
%Although ERS (without batch communication) approaches the result of PML as \( N \to \infty \), it is not sample-efficient in this case. This is because, after receiving the hash value \( V_K \) from the encoder, the decoder only retains approximately \( \mathrm{V}^{-1} \) samples per batch, which potentially lowers the acceptance probability on the decoder side and as the result, decrease the matching probability. On the other hand, we observe that the batch communication version is much effective in this setting.
%\end{remark}


==> old/ERS_old.tex <==
\newpage

\vspace{-4pt}\section{Ensemble Rejection Sampling}\vspace{-4pt}
We show that ERS\cite{deligiannidis2020ensemble}, an exact sampling scheme that combine RS with IS,  can improve the matching probability and maintain a coding cost close to the theoretical optimum in channel simulation. 

\vspace{-3pt}
\subsection{Background}\label{sec:background_ers}

 \textbf{Setup and Definitions.} We begin by defining the common randomness $W$, which includes a set of  exponential random variables to employ the Gumbel-Max trick for IS \cite{phan2024importance,theis2022algorithms}, i.e.:
\begin{align}
    W &= \{ (B_1, U_1), (B_2, U_2), ...\}, \text{ where } U_i \sim  \mathcal{U}(0,1)\\
    {B}_i&=\{(Y_{i1}, S_{i1}), (Y_{i2}, S_{i2}),..., (Y_{iN}, S_{iN})\}, \text{ where } Y_{ij} \sim P_Y(.), S_{ij} \sim \mathrm{Exp}(1),
\end{align}
where we refer to each $B_i$ as a batch. A selected sample $Y_K$ from $W$ is defined by two indices: the \textit{batch index} \( K_1 \)  and the \textit{local index} in \( B_{K_1} \), denoted as \( K_2 \). Its \textit{global index} within $W$ is $K$, where:
\begin{align}
    K= (N-1)K_1 + K_2 \label{index_ERS},
\end{align}
and we write $Y_K \triangleq Y_{K_1,K_2}$. Note that $K, K_1, K_2$ are random variables. %In the coupling setting, where each party selects its own sample, we use subscripts to indicate ownership of each index. Specifically, \(K_A\), \(K_{1,A}\), and \(K_{2,A}\) denote the global, batch, and local indices selected by party \(A\), respectively.

\textbf{Sample Selection.} Consider the target distribution $P_{Y|X}(.|x)$, for each batch $B_i$ within $W$, the ERS algorithm  selects a candidate index $K^{\mathrm{cand}}_i$ and decides to whether accept/reject $Y_{K^{\mathrm{cand}}_i}$ based on $U_i$. This process ensures that the accepted  \( Y_{K} {\sim} P_{Y|X}(\cdot | x) \) and is denoted for simplicity as as:
\begin{equation}
    K = \mathrm{ERS}(W; P_{Y|X}, P_Y), \label{ers_selection}
\end{equation}
which consists of an importance sampling step followed by acceptance/rejection:
\begin{itemize}
    \item \textit{Step 1 (Gumbel-Max IS):} We select a candidate index \(K^{\mathrm{cand}}_i\) using the Gumbel-Max trick as follows:
\begin{align}
    K^{\mathrm{cand}}_i = \operatorname*{argmin}_{1 \leq k \leq N} \frac{S_{ik}}{\lambda_{ik}}, \quad \text{where} \quad \lambda_{ik} = \frac{P_{Y|X}(Y_{ik}|x)/P_Y(Y_{ik})}{\sum_{j=1}^N P_{Y|X}(Y_{ij}|x)/P_Y(Y_{ij})}.
\end{align}
This corresponds to applying the Gumbel-Max trick to the normalized importance weights \(\vec{\lambda}_i = (\lambda_{i1}, \dots, \lambda_{iN})\). For convenience, we denote this selection process as:
\begin{equation}
    K^{\mathrm{cand}}_i = \mathrm{Gumbel}(B_i; P_{Y|X=x}, P_Y). \label{gumbel_selection}
\end{equation}

\item \textit{Step 2 (Rejection/Acceptance): } We decide to accept $Y_{K^{\mathrm{cand}}_i}$ if $ U_i \leq \frac{\hat{Z}(Y_{i,1:N})}{\bar{Z}(Y_{i,1:N}, K^{\mathrm{cand}}_i)}$, where
\begin{align*}
   \hat{Z}(Y_{i,1:N}) {=} \sum^N_{j=1} \frac{P_{Y|X}(Y_{ij}|x)}{P_Y(Y_{ij})} , \quad \bar{Z}(Y_{i,1:N}, K^{\mathrm{cand}}_i){=} \sum_{\substack{j=1 \\ j\neq K^{\mathrm{cand}}_i}}^N \frac{P_{Y|X}(Y_{ij}|x)}{P_Y(Y_{ij})} {+} \omega,
\end{align*}
and $\omega$ is as in (\ref{define_omega}). If $K^{\mathrm{cand}}_i$ (and  batch $B_i$) is accepted, we  set $K_1=i$, $ K_2=K^{\mathrm{cand}}_i$, $K=(N{-}1)1i + K^{\mathrm{cand}}_i$ and return $Y_K$. Otherwise, we repeat the process with batch $B_{i+1}$.
\end{itemize}


We provide the connection between ERS and RS in Appendix \ref{prelim}. Note that the target and proposal distributions to be any, e.g., replacing $P_Y$ with $Q_Y$, as long as the bounding condition holds. Let the batch average acceptance probability as $\Delta$ and we have $\Delta \xrightarrow[]{} 1.0$ as $N \xrightarrow[]{} \infty$. Finally, we define:
\begin{equation}
    N^* = N\Delta^{-1},
\end{equation}
as the average number of proposals (or runtime) required for ERS. 
%Without step 2, the output samples (by IS) will be biased, albeit reducible by increasing the batch size \( N \).


%where:
%\begin{align}
%    \hat{Z}(Y^N_1) = \sum^N_{j=1} \frac{P_{Y|X}(Y_{ij}|x)}{P_Y(Y_{ij})} , \quad \bar{Z}_i(Y^N_1, \Tilde{K}_i)= \sum_{\substack{j=1 \\ j\neq \Tilde{K}_i}}^N \frac{P_{Y|X}(Y_{ij}|x)}{P_Y(Y_{ij})} + \omega, 
%\end{align}

%\begin{remark}\label{remark_ers}We  note that the ERS can be considered as a standard RS on the following \textit{batch proposal distribution} $\bar{Q}_{Y^N_1,K}(y^N_1, k)$ and \textit{target distribution} $\bar{P}_{Y^N_1,K}(y^N_1, k)$:
%\begin{align}
    %\bar{Q}_{Y^N_1,K}(y^N_1, k) 
    %&{=} \frac{P_{Y|X}(y_k|x)}{\hat{Z}(y^N_1)}\prod^N_{\substack{j=1 \\ j\neq k}}P_Y(y_j)  ,\quad \bar{P}_{Y^N_1,K}(y^N_1, k){=} \frac{P_{Y|X}(y_k|x)}{\Delta\bar{Z}(y^N_1,k)}\prod^N_{\substack{j=1 \\ j\neq k}}P_Y(y_j) ,
%\end{align}
%where $\Delta$ is  the batch average acceptance probability and $\Delta \xrightarrow[]{} 1.0$ as $N \xrightarrow[]{} \infty$. 
%\begin{align}
%    \Delta &= 
%    \mathbb{E}_{Y^N_1 \sim P_Y(.)}\left[\frac{N}{\bar{Z}(1, Y^N_1)}\right] \geq \frac{N}{\mathbb{E}_{Y^N_1 \sim P_Y(.)}[\bar{Z}(1)]}= \frac{N}{N-1+\omega}
%\end{align}
%where the last inequality indicates that the probability of accepting a batch increase with its size $N$.
%\end{remark}



%\begin{wrapfigure}{R}{0.45\textwidth}
%\begin{minipage}[t]{0.45\textwidth}
%\begin{algorithm}[H]
%\caption{Ensemble Rejection Sampling}\label{alg:ers}
%\begin{algorithmic}
    
%        \State Sample $Y_1,Y_2,...,Y_N \sim Q_Y(.)$
%        \State Compute $\lambda_1,\lambda_2,...,\lambda_N$
%        \State
        
%        \State 
%        \State
%    \State Entropy-code 
%\end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\end{wrapfigure}
\vspace{-3pt}
\subsection{Channel Simmulation with ERS}\label{ers_coding_cost}\vspace{-3pt}
 %We first define the following terminology in Figure \ref{fig:ers_coding} (left). 

For $N=1$, ERS becomes the standard RS and thus achieves the coding cost shown in Proposition \ref{prop:coding_RS}. On the other hand, as $N\xrightarrow{} \infty$, we have the batch acceptance probability $\Delta\xrightarrow[]{} 1.0$, meaning that we almost always accept the first batch and thus the coding cost is similar to the one in IS schemes \cite{phan2024importance,theis2022algorithms}, which follows (\ref{com_cost_1}). This section presents the result for general \(N\), which is more challenging to establish due to the appearance of inverse sums of ratio terms, similar to those encountered in self-normalized IS \cite{agapiou2017importance}.

\begin{figure*}[t]%
    \centering%
    \vspace{-18pt}
    \hspace{-5mm}
    \begin{subfigure}[t]{0.48\linewidth}%
        \includegraphics[width=\linewidth]{Neurips2025/figures/ERS Coding_3.pdf}%
    \end{subfigure}%
    %\hspace{3mm}
    \begin{subfigure}[t]{0.55\linewidth}%
        \includegraphics[width=\linewidth]{Neurips2025/figures/ERS_coding_N.pdf}%
    \end{subfigure}%
    \vspace{-5pt}
    \caption{\textit{Left}: Illustration of ERS Coding. \textit{Right}: Empirical results comparing the combined coding cost of $\hat{K}_1, \hat{K}_2$ with their associated theoretical upper-bound. Both figures use $P_Y(.)=\mathcal{N}(0,1.0)$, where the first figure varies $P_{Y|X}(.|x) = \mathcal{N}(1.0, \sigma^2)$ with \(\sigma^2 \in [1 \times 10^{-4}, 5 \times 10^{-3}]\) and the second one fixes $\sigma^2=10^{-3}$ while varying the batch size $N$.}
     \label{fig:ers_coding}
     \vspace{-14pt}
\end{figure*}
%\footnote{From this perspective, the motivation for the Sorting Method in Section \ref{rs_coding_cost} becomes clear: since the decoder does not have access to the batch proposal distribution \( \bar{Q}_{Y^N_1,K}(y^N_1, k) \), it is not feasible to use the Binning Method.} 


\textbf{Encoding Scheme. } We view the selection of $K_1$  as a rejection sampling process on a whole batch (see Appendix \ref{prelim}) and apply the Sorting Method to encode $K_1$. Specifically, we collect every $\lfloor \Delta^{-1}\rfloor$ batches into one \textit{group of batches}, send the group index and the rank of  $U_{K_1}$ within this group. For the local index $K_2$, we use the Gumbel-Max Coding approach \cite{phan2024importance}, see Figure \ref{fig:ers_coding} (left). In particular:
\begin{itemize}
    \item Encoding $K_1$: we represent $K_1$ by two messages $L$ and $\hat{K}_1$.  Here, $L$ is the index of group of batches $K_1$ belongs to and $\hat{K}_1$  is the rank of $U_{K_1}$ within this group, i.e.,  we sort the list:$$U_{\phi(1)}\leq U_{\phi(2)}\leq...\leq U_{\phi(\lfloor \Delta^{-1}\rfloor)}$$ within the $L^{\mathrm{th}}$ group  and send the rank $\hat{K}_1$ of $U_{K_1}$ within this group, i.e. $\phi(\hat{K}_1)=K_1$. 
    \item Encoding $K_2$: We first sort the exponential random variables within the selected batch $K_1$, i.e. $S_{\pi(1)} \leq S_{\pi(2)} \leq ...\leq S_{\pi(N)}$ and send the rank $\hat{K}_2$ of $S_{K_2}$, i.e. $\pi(\hat{K}_2){=}K_2$, as in \cite{phan2024importance}.
\end{itemize}
\textbf{Coding Cost.} We outline the main results for the coding costs, details in Appendix \ref{analysis_ers}. Specifically:
\begin{equation}
       \mathbb{E}[\log L] \leq 1 \text{ bit }, \quad\mathcal{K} = \mathbb{E}[\log \hat{K}_1] + \mathbb{E}[\log \hat{K}_2]\leq D_{KL}(P_{Y|X}(.|x)||P_Y(.)) {+}  2\log(e) {+} 3 \text{ bits}, \notag
    \end{equation}
where the second bound is one of the core technical contributions of this work. We empirically validate the bound on $\mathcal{K}$  in Figure \ref{fig:ers_coding}(right).   Proposition \ref{prop:coding_ERS} shows the overall coding cost for $K$:

 %Similarly, for $\hat{K}_1$, we have:
%\begin{align}
%    \mathbb{E}[\log \hat{K}_1] \leq D_{KL}(\bar{P}_{Y^N_1,K}(.)|| \bar{Q}_{Y^N_1,K}(.)) + \log(e)
%\end{align}
%$\mathbb{E}[\hat{K}_1]$ is upperbound by $D_{KL}(\bar{P}_{Y^N_1,K}(.)|| \bar{Q}_{Y^N_1,K}(.)) + \log(e)$, which is equivalent to:
%    \begin{align}
%        \mathbb{E}[\log \hat{K}_1] \leq  \mathbb{E}_{Y^N_1 \sim P_Y(.)} \left[\frac{NP_{Y|X}(Y_1|x)}{\Delta\bar{Z}(Y^N_1,1)P_Y(Y_1)}\log\left(\frac{\hat{Z}(Y^N_1)}{\Delta\bar{Z}(Y^N_1,1)}\right)\right] + \log(e)   
%    \end{align}
%Finally, for $\hat{K}_2$, we have:
%    \begin{align}
%        \mathbb{E}[\log(\hat{K}_2)] \leq \mathbb{E}_{Y^N_1 \sim P_Y(.)}\left[\frac{NP_{Y|X}(Y_1|x)}{P_Y(Y_1)\Delta \bar{Z}(Y^N_1,1)} \log \left(\frac{NP_{Y|X}(Y_1|x)}{P_Y(Y_1)\hat{Z}(Y^N_1)}\right)\right] + \log(e) 
%    \end{align}

%Although $\mathbb{E}[\log \hat{K}_1]$ and $\mathbb{E}[\log \hat{K}_2]$ look complicated, we (informally) observe that:

%\begin{align}
%    \mathcal{K}  &{\leq}  D_{KL}(P_{Y|X}(.|x)||P_Y(.)) {+} 2\log(e) {+} \mathbb{E}_{Y_{1:N} \sim P_Y(.)} \left[\frac{N}{\Delta\bar{Z}(Y_{1:N},1)}\log\left(\frac{N}{\Delta\bar{Z}(Y_{1:N},1)}\right)\right] \label{special_ineq_main} \\
%    & {\leq} D_{KL}(P_{Y|X}(.|x)||P_Y(.)) {+}  2\log(e) {+} 3 ,
%\end{align}
%where bounding the expectation term in \eqref{special_ineq_main} by a constant $3$ is one of the core technical contributions of this work. We experimentally validate the bound on $\mathcal{K}$ and show this in Figure \ref{fig:ers_coding}(right).  Following these results, Proposition \ref{prop:coding_ERS} shows the overall coding cost for $K$:

\begin{proposition} \label{prop:coding_ERS} Given $(X,Y)\sim P_{X,Y}$ and $K$  defined as above. For any batch size $N$, we have:
\begin{equation}
    R \leq {H}[K|W] +1 \leq I(X;Y) + 2\log(I(X;Y) + 8) + 10, \label{eq:rejection_coding_cost_ERS}
\end{equation}    
\end{proposition}\begin{proof}
    See Appendix  \ref{ers_coding_cost_proof}.
\end{proof}
This concludes the coding cost of ERS, which is a new channel simulation method beside PFR and GRS that achieves a bound close to the theoretical minimum.

==> old/intro_old.tex <==
\section{Introduction}\label{intro}
%\begin{wrapfigure}{r}{0.35\textwidth}
%\vspace{-10pt}
%    \centering
%    \includegraphics[width=0.35\textwidth]{Neurips2025/figures/rs_binning.pdf}
%    \vspace{-20pt}
%    \caption{Binning Method for RS.}
%    \label{fig:rs_bin}
%    \vspace{-10pt}
%\end{wrapfigure}
One-shot channel simulation is a task of efficiently compressing a finite blocklength of noisy samples. Specifically, this can be described as a two-party communication problem where the encoder obtains a sample $X \sim P_X$ and wants to transmit its noisy version $Y \sim P_{Y|X}$ to the decoder, with the communication efficiency measured by the coding cost $R$ (bits/sample).  Assuming both parties share access to a common randomness source \( W \), the encoder applies a Monte Carlo procedure to select a candidate from \( W \) that satisfies the desired distributional constraints. It then encodes this candidate into a binary string $\mathcal{M}\in \{0,1\}^*$ with length $\ell(\mathcal{M})$, aiming to achieve the cost $R$ that satisfies:\begin{equation}
 R \leq I(X;Y) + c_1\log(I(X;Y)+c_2) + c_3 , \label{com_cost_1}
\end{equation}
where we note that \( R = \mathbb{E}[\ell(\mathcal{M})] \)  and \( I(X;Y) \) is the mutual information between \( X \) and \( Y \), which represents the theoretical optimal solution attainable in the asymptotic (i.e., infinite blocklength) setting \cite{cuff2013distributed} (also see Figure 1 (left)). Different techniques may yield slightly different coding costs, characterized by the positive constants \( c_1, c_2, \) and \( c_3 \)\cite{harsha2007communication,li2024pointwise}, but any approach that fails to achieve the leading term \( I(X;Y) \) is generally considered inefficient. Since the conditional distribution $P_{Y|X}$ can be designed to target different objectives, channel simulation is a generalized version of lossy compression. As a result, it has been widely adopted in various machine learning tasks such as data/model compression \cite{agustsson2020universally, blau2019rethinking, yang2025progressive, havasi2019minimal}, differential privacy \cite{shah2022optimal, triastcyn2021dp},  and federated learning \cite{isik2024adaptive}.


While much of the prior work has focused on the point-to-point setting above, recent works have extended channel simulation techniques to more complex distributed compression scenarios \cite{li2021unified,phan2024importance}. For these applications, we consider the following canonical setting, illustrated in Figure 1 (right),  which slightly differs from previous point-to-point communication setup: the encoder (party \(A\)) and decoder (party \(B\)) aim to sample \(Y_A\) and \(Y_B\) from their respective target distributions, denoted by \(P^A_Y(\cdot)\) and \(P^B_Y(\cdot)\), using shared randomness \(W\). Here, we are interested in the \textit{distributed matching probability}, i.e. the probability that both parties select the same value, which is non-negligible as the selection process is coupled through $W$. Using this matching probability, we can design an efficient communication scheme for distributed compression scenarios, such as the Wyner-Ziv setup \cite{wyner1976rate} where the decoder can access side information unavailable to the encoder \cite{phan2024importance}. 

%\begin{figure*}[t]%
%    \centering%
%    \vspace{-15pt}
%    \hspace{-10mm}
%    \begin{subfigure}[t]{0.4\linewidth}%
%        \includegraphics[width=\linewidth]{Neurips2025/figures/ChanSim.pdf}%
%    \end{subfigure}%
%    \hspace{10mm}
%    \begin{subfigure}[t]{0.4\linewidth}%
%        \includegraphics[width=\linewidth]{Neurips2025/figures/Distributed Matching (1).pdf}%
%    \end{subfigure}%
%    \vspace{-3pt}
%    \caption{(Left) \textit{Channel Simulation}: the encoder aims to send a message $\mathcal{M}$ with rate close to theoretical optimal $I(X;Y)$ such that the decoder retrieve sthe correct sample following $P_{Y|X}(.|x)$. Visual illustration of (Left) \textit{Channel Simulation} where the encoder aims to send a message $\mathcal{M}$ with rate close to theoretical optimal $I(X;Y)$ such that the decoder retrieve. }
%     \label{fig:visualizations}
%     \vspace{-10pt}
%\end{figure*}

\begin{figure*}[t]%
    \centering%
    \vspace{-21pt}
        \includegraphics[width=1.0\linewidth]{Neurips2025/figures/Illu2.pdf}%
    \vspace{-3pt}
    \caption{\textit{Left}: Channel simulation setup.  \textit{Middle}: Distributed matching and Distributed compression (with dashed line) setup. In the latter, the decoder receives a private side information $X'$ and messages from the encoder to improve the matching probability. \textit{Right}: visualization of the communication scheme in Section \ref{wyner_ziv}.}
    %\caption{\textit{Left}: \textit{Channel Simulation}: the message $\mathcal{M}$ is compressed with rate close to theoretical optimal $I(X;Y)$ while ensuring the decoder obtains $Y {\sim} P_{Y|X}(.|x)$.  (\textit{Middle}) \textit{Distributed Matching}: we want to design a selection rule to increase the probability $Y_A=Y_B$. For distributed compression (with the dashed lines), the decoder receives a private side information $X'$ and messages from the encoder (see the next figure) to improve the matching probability. (\textit{Right}) \textit{Distributed Compression Protocol}: visualization of the communication scheme in Section \ref{wyner_ziv}.}
     \label{fig:visualizations}
     \vspace{-12pt}
\end{figure*}

Currently, Poisson Monte Carlo (PMC) \cite{maddison2016poisson} and importance sampling (IS) are the two main Monte Carlo methods being applied across both scenarios\cite{li2024channel}. Particularly, the Poisson Functional Representation Lemma (PFRL)\cite{li2018strong} provides a near-optimal coding cost in ~\eqref{com_cost_1} for channel simulation. The Poisson Matching Lemma (PML) \cite{li2021unified} was later developed for distributed matching scenarios, enabling the analysis of achievable error rates in various compression settings. However, PMC requires an infinite number of proposals and cannot guarantee termination when certain conditions on the distributions are unknown or not satisfied. This often arises in practical distributed compression scenarios when the density function of \( P^B_Y \) is estimated via machine learning. IS-based approaches, including the importance matching lemma (IML) for distributed compression \cite{phan2024importance}, bypass this issue by limiting the number of proposals in $W$ to be finite. Yet, the output distribution from IS is biased \cite{havasi2019minimal,theis2022algorithms}, and thus not favorable in certain applications such as differential privacy \cite{liu2024universal}. It is hence interesting to see whether a new Monte Carlo scheme and coding method can be developed to handle both scenarios without compromising sample quality or termination guarantees. 

%In this work, we develop new channel simulation and distributed matching results based on Ensemble Rejection Sampling (ERS)

%One particular class of sampling schemes that has been overlooked is rejection sampling (RS), which—despite being one of the earliest one-shot channel simulation techniques \cite{steiner2000towards}—is widely regarded as inefficient \cite{theis2022algorithms}. 

This work studies rejection sampling schemes and its applicability to these two scenarios. We begin by revisiting and improving the coding efficiency of standard rejection sampling (RS) in channel simulation \cite{steiner2000towards, theis2022algorithms}. In particular, we introduce a new coding scheme based on sorting that attains an entropy bound comparable to ~\eqref{com_cost_1}, extending the prior achievability result by \citet{braverman2014public} for discrete distributions to broader settings, while employing a distinct mechanism. However, our analysis also suggests that the distributed matching probabilities of both RS and its adaptive variant, namely greedy rejection sampling (GRS)\cite{flamich2023adaptive}, are lower than that of the PML, making them less suitable for distributed compression. Interestingly, by combining RS with IS—a technique known as \emph{Ensemble Rejection Sampling} (ERS)~\cite{deligiannidis2020ensemble}—one can improve the distributed matching probability without degrading the sample quality. We demonstrate, with provable guarantees, that ERS retains efficient coding performance in channel simulation and further introduce \textcolor{red}{a new technique that bypasses the termination issue in distributed compression.}

In summary, our contribution is as follows:
\begin{enumerate}
    \item We propose a sorting-based compression method for RS that achieves the coding cost near the theoretical optimum \( I(X;Y) \). Our further analysis indicates that its distributed matching probability is less competitive to ones obtained by PMC and IS-based approaches.
    \item Using the analysis in RS and previous results in IS, we develop an efficient coding scheme for channel simulation with ERS. We provide a theoretical analysis to bound its distributed matching probability, showing the improvement over standard RS. 
    \item  We introduce a new coding scheme based on ERS distributed matching results for distributed compression that bypass the termination issue in practical scenario.
    \item  We conduct experiments on synthetic Gaussian source, distributed compression with MNIST and vertical federated learning with CIFAR-10 to validate our approach.
\end{enumerate}


==> old/note_RS_old.tex <==
\section{Rejection Sampling}
This section reviews the existing coding scheme of standard RS ,  pointing out its source of inefficiency, and introduces a new technique that achieves a bound comparable to (\ref{com_cost_1}). Finally, we discuss results on matching probability bounds for standard RS (and GRS), showing that they are less competitive compared to PML and IML. %For both scenarios, we also discuss the performance of greedy rejection sampling (GRS) and its implications.

%\subsection{Rejection Sampling (RS)}
\subsection{Coding Cost}\label{rs_coding_cost}

\textbf{Runtime-Based Coding Cost of RS. }
Let $X \sim P_X$ be the input to the encoder, who aims to transmit a sample $Y \sim P_{Y|X}(\cdot | X)$ to the decoder. The marginal distribution $P_Y(\cdot)$ serves as the proposal distribution, also known by the decoder, and satisfies the following \textit{bounding condition} i.e.,  
\begin{align}
    \max_{x,y} ({P_{Y|X}(y|x)}{P^{-1}_Y(y)}) \leq \omega, \text{ for some } \omega \geq 1 \label{define_omega}, 
\end{align}
We define the common randomness $W$ shared between two parties:
$
W = \{(Y_1, U_1), (Y_2, U_2), \dots\},
$
where each $Y_i$ is drawn i.i.d. from $P_Y(\cdot)$, and each $U_i$ is drawn i.i.d. from the standard uniform distribution $\mathcal{U}(0,1)$. Given $X=x$, the encoder picks the first index $K$ such that:
\begin{equation}
 U_{K} \leq \frac{P_{Y|X}(Y_{K}|x)}{\omega P_Y(Y_{K})} \label{equation_rs}
\end{equation}
which gives us $Y_{K}\sim P_{Y|X}(.|x)$. For each individual sample $Y_i$, the acceptance probability is: $$\Pr(\text{Accept}) = {\omega}^{-1},$$
and hence, we can compress $K$ with a coding cost of: 
\begin{equation}
    R \leq H[K] + 1\leq \log(\omega) + 2, \label{RS_naive}
\end{equation}
which is inefficient compared to $I(X;Y)$.  For this reason, GRS, whose runtime entropy $H[K]$ achieves the desired bound, is considered a better approach for channel simulation, but with practical limitations as discussed in Section \ref{intro}. 

Before introducing our approach, we note that the above coding scheme does not leverage the common randomness \(W\) shared between the encoder and the decoder \cite{li2024channel}. This means a tighter upper bound on the rate $R$ can be obtained with the conditional entropy \(H[K | W]\) instead of \(H[K]\). 

%ne might note that the bound in (\ref{RS_naive}) seems to contradict prior work by \citet{braverman2014public}, which demonstrates that RS can achieve a similar bound to (\ref{com_cost_1}) for discrete distributions. The key difference lies in the fact that the coding cost above 


\textbf{Coding Technique. } Our new coding scheme achieves a bound similar to (\ref{com_cost_1}) by  performing sorting on the uniform random variables and is thus referred to as the \textit{Sorting Method}. Assume that the encoder and decoder agree on the value of \(\omega\) prior to communication, we first collect every \(\lfloor\omega\rfloor\) proposals into one group, ( $\lfloor.\rfloor, \lceil.\rceil$ are floor and ceil functions respectively). We encode two messages: one for the group index $L$ and one for the rank $\hat{K}$ of the selected \(U_K\) within that group, in particular: %Interestingly, this scheme does not require the decoder to have access to the proposal distribution \( P_Y(\cdot) \), which will later be shown to be useful in the context of Ensemble Rejection Sampling (ERS) in Section \ref{ers_coding_cost}. We assume that the encoder and decoder agree on the value of \(\omega\) prior to communication.

%\textit{Binning Method. } For each pair $(U_i,Y_i)$ from $W$, we denote $\tilde{U}_i=\omega U_i P_Y(Y_i)$. The central idea of this method is to send the bin index of the first accepted sample, where the bin corresponds to the smallest scaled region that $\tilde{U}_K$ belongs to, visualized in Figure \ref{fig:rs_bin}. The encoding process consists of two steps where  we encode $K$ into two separate messages:
%\begin{enumerate}
%    \item \textit{Binning.} The bin $T= \lceil \frac{\tilde{U}_{K}}{P_Y(Y_{K})}\rceil$, i.e. $T=3$ in the case of Figure \ref{fig:rs_bin}. After sending $T$, both parties assort the following set:
%    \begin{equation}
%        \mathcal{S}_T = \{i | (T-1)P_Y(Y_i) \leq \tilde{U}_i \leq TP_Y(Y_i)\},
%    \end{equation}
%    i.e. remove all the proposals that are not within the range of the selected candidates. Also: 
%    \begin{equation}
%        \mathbb{E}[\log T] \leq D_{KL}(P_{Y|X}(.|x)||P_Y(.)) + \log(e) \text{ bits}
%    \end{equation}
%    \item \textit{Index Selection.} The encoder locates the original chosen index $K$ within $\mathcal{S}_T$, says $G$, and send $G$ to the receiver. In Figure \ref{fig:rs_bin}, we have $G=3$, corresponds to $(Y_7, U_7)$ in the original $W$. In general, we have: 
%    \begin{equation}
%        \mathbb{E}[\log G] \leq 1 \text{ bit}
%    \end{equation}
%\end{enumerate}

\begin{figure*}[t]%
    \centering%
    \vspace{-0.5cm}
    \hspace{-10mm}
    \begin{subfigure}[t]{0.45\linewidth}%
        \includegraphics[width=\linewidth]{Neurips2025/figures/RS_Sort_v3.pdf}%
    \end{subfigure}%
    \hspace{3mm}
    \begin{subfigure}[t]{0.26\linewidth}%
        \includegraphics[width=\linewidth]{Neurips2025/figures/ElogL.pdf}%
        %\caption{Level 2 uncertainty.}%
    \end{subfigure}%
    \hspace{-2mm}
    %trim={1.5cm 1.5cm -0.5cm 0.5cm}
    \begin{subfigure}[t]{0.26\linewidth}%
        \includegraphics[width=\linewidth]{Neurips2025/figures/ElogKhat.pdf}%
    \end{subfigure}%
    \vspace{-2pt}
    \caption{\textit{Left}: Visualization of our Sorting Method for Standard RS. \textit{Right}: Empirical results comparing $\mathbb{E}[\log(L)]$ and $\mathbb{E}[\log(\hat{K})]$ with their associated theoretical upper-bound across different target distribution. We use $P_Y(.)=\mathcal{N}(0,1.0)$ and $P_{Y|X}(.|x) = \mathcal{N}(1.0, \sigma^2)$ where $\sigma^2 \in [0.01, 0.1]$.}
     \label{fig:sort_method}
     \vspace{-10pt}
\end{figure*}

\begin{enumerate}
    \item \textit{Encoding $L$}: The encoder sends the ceiling $L  = \lceil \frac{K}{\lfloor\omega\rfloor}\rceil $, i.e. $L=2$ in Figure \ref{fig:sort_method} (left). The decoder then knows  $(L-1)\lfloor\omega\rfloor + 1 \leq K \leq L\lfloor\omega\rfloor$, i.e. $K$ is in group $L$. 
    \item \textit{Encoding $\hat{K}$}: The encoder and decoder both sort the uniform random variables $U_i$ within the selected group $(L-1)\lfloor\omega\rfloor + 1 \leq i \leq L\lfloor\omega\rfloor$, i.e. $$U_{\pi(1)} \leq U_{\pi(2)} \leq ...\leq U_{\pi(\lfloor \omega\rfloor)}$$ where $\pi(.)$ maps the sorted indices with the original ones. The encoder sends the rank of $U_{K}$ within this list, i.e. sends the value $\hat{K}$ such that $K=\pi(\hat{K})$, which the decoder uses to retrieve $Y_{K}$ accordingly. This corresponds to $\hat{K}=2$ in Figure \ref{fig:sort_method} (Left). 
\end{enumerate}
\textbf{Coding Cost.} In terms of the coding cost at each step, i.e., $\mathbb{E}[\log L]$ and $\mathbb{E}[\log \hat{K}]$, we have:
    \begin{equation}
        \mathbb{E}[\log L] \leq 1 \text{ bit }, \quad \mathbb{E}[\log \hat{K}] \leq D_{KL}(P_{Y|X}(.|x)||P_Y(.)) + \log (e) \text{ bits},
    \end{equation}
where Figure \ref{fig:sort_method} (right) shows the empirical results verifying the bounds. The proof for these bounds are shown in Appendeix \ref{sort_proof}. We then perform entropy coding for each message separately using Zipf's distribution and prefix-free coding. Proposition \ref{prop:coding_RS} shows their overall coding cost:

\begin{proposition} \label{prop:coding_RS} Given $(X,Y)\sim P_{X,Y}$ and $K$  defined as above. Then we have:
\begin{equation}
    R \leq {H}[K|W] +1 \leq I(X;Y) + \log(I(X;Y) + 1) + 8, \label{eq:rejection_coding_cost}
\end{equation}    
\end{proposition}\begin{proof}
    See Appendix  \ref{rej_coding_final}.
\end{proof}
%We conclude this discussion with a note that the constant in (\ref{eq:rejection_coding_cost}) is slightly higher than the bound in (\ref{com_cost_1}), due to the coding cost of $G$ and $T$ in the {Sorting Method} and {Binning Method} respectively, as some extra bits are required for the joint messages to be uniquely decodable.

%Interestingly, this scheme does not require the decoder to have access to the proposal distribution \( P_Y(\cdot) \), which will later be shown to be useful in the context of Ensemble Rejection Sampling (ERS) in Section \ref{ers_coding_cost}. 

We note that the approach of \citet{braverman2014public} for discrete distributions can be extended to the continuous case, included in Appendix~\ref{binning_proof} for completeness. Our mechanism, however, is fundamentally different: it does not require the decoder to have knowledge about the proposal distribution \( P_Y(\cdot) \). This distinction is particularly important in the ERS setting of Section~\ref{ers_coding_cost}, where incorporating the method of \citet{braverman2014public} is nontrivial.


%\begin{remark}\label{remark_omega}
%    Note that this scheme can be extended if the encoder wishes to use the constant $\Tilde{\omega}=\max_{y} {P_{Y|X}(y|x)}/{P_Y(y)}$ instead of $\omega$ for the rejection/acceptance step (but the chunk size remains ${\lfloor\omega\rfloor}$). The coding cost remains similar with a slight change in the constants.
%\end{remark}

    
\subsection{Distributed Matching} \label{sec:rs_distributed_matching}
%We establish matching probability bounds of the event two parties selecting the same index from the same shared randomness $W$ using RS.
 
 Let \( P^A_Y \) and \( P^B_Y \) denote the target distributions of party \( A \) and \( B \), respectively. Each party independently performs RS using the proposal distribution \( Q_Y(\cdot) \) to select indices \( K_A \) and \( K_B \). We assume the bounding condition holds for both parties, i.e.  
$
\max_y\left({P^A_Y(y)}{Q^{-1}_Y(y)}, {P^B_Y(y)}{Q^{-1}_Y(y)}\right) \leq \omega,
$
Proposition \ref{prop:match_RS} shows the probability that they select the same index, given that \( Y_{K_A} = y \).
\begin{proposition} \label{prop:match_RS} Let $W, Q(.), P^A_Y(.)$ and $P^B_Y(.)$ defined as above. Then we have:
\begin{equation}
    \Pr(Y_{K_{A}} = Y_{K_{B}}| Y_{K_{A}} = y ) = \frac{\min (1, P^B_Y(y)/P^A_Y(y))}{1 + \mathrm{TV}(P^A_Y, P^B_Y)} \geq \frac{1}{2\left(1 + P^A_Y(y)/P^B_Y(y)\right)}
\end{equation}    
%Furthermore, we have:
%\begin{align}
%    \Pr(Y_{K_{A}} = Y_{K_{B}}) = \frac{1-\mathrm{TV}(P^A_Y, P^B_Y)}{1+ \mathrm{TV}(P^A_Y, P^B_Y)}.
%\end{align}
where $\mathrm{TV}(P^A_Y, P^B_Y)$ is the total variation distance between two distribution $P^A_Y$ and $ P^B_Y$.
\end{proposition}
\begin{proof}
    See Appendix \ref{match_RS}.
\end{proof}This matching probability is not as strong, compared to PML, details in Appendix \ref{compare_possion}\footnote{\citet{daliri2024coupling} also arrives to a similar conclusion but for discrete case, targeting a different problem.}. Compared to IML, since IML approaches PML for a large enough number of proposals, the same conclusion also applies. In the case of GRS, we provide an analysis via a non-trivial example in Appendix \ref{GRS_match}, where we demonstrate that it is possible to construct target and proposal distributions such that $\Pr(K_A {=} K_B\mid Y_{K_A} {=} y) \to 0.0$, even when $P^A_Y(y) = P^B_Y(y)$. In contrast, this probability is greater than $1/4$ for standard RS. In summary, while GRS and RS can achieve a coding cost in (\ref{com_cost_1}), its matching probability remains lower than that attainable by PML and IML.

%. In the case all distributions are discrete,  one can show that the matching probabily of PML is greater than the equality shown in Proposition \ref{prop:match_RS}, i.e. see \cite{daliri2024coupling}. 

==> proof_batch_commu_uncond.tex <==
\subsection{Proof of Proposition \ref{prop:match_ers_comm}}
We now formally prove the bound  Proposition \ref{prop:match_ers_comm}. Recall that $K_{2,A}$ is the sample index within the selected batch of $A$ and let $\Tilde{Y}^N_1$ be the samples within the selected batch by the encoder (party $A$), we have:
\begin{align}
    &\Pr(Y_{K_A} = Y_{\Tilde{K}_B}|Y_{K_A} = y_1) \\
    &\geq \Pr(K_{2,A} = {\Tilde{K}_B}|Y_{K_A} = y_1) \\
    &= \sum^N_{i=1}\Pr(K_{2,A} = {\Tilde{K}_B}=i|Y_{K_A} = y_1) \\
    &= N\Pr(K_{2,A} = {\Tilde{K}_B}=1|Y_{K_A} = y_1) \quad \text{ (Due to Symmetry)} \\
    &= N\Pr(K_{2,A} = {\Tilde{K}_B}|Y_{K_A} = y_1, K_{2,A} =1) \Pr(K_{2,A} =1|Y_{K_A} = y_1) \\
    &= \Pr(K_{2,A} = {\Tilde{K}_B}|Y_{K_A} = y_1, K_{2,A} =1) \quad \text{(Since: } \Pr(K_{2,A} =1|Y_{K_A} = y_1)=N^{-1}) \\
    &=\int^{\infty}_{-\infty} P(\Tilde{Y}^N_2=y^N_2| Y_{K_A}=y_1, K_{2,A} = 1) \Pr(K_{2,A} = \Tilde{K}_B|Y_{K_A}=y_1, K_{2,A}=1, \Tilde{Y}^N_2=y^N_2) dy^N_2,
\end{align}
We now note that:
\begin{align}
    &\Pr(K_{2,A} = \Tilde{K}_B|Y_{K_A}=y_1, K_{2,A}=1, \Tilde{Y}^N_2=y^N_2)\\ &= \Pr(K_{2,A} = \Tilde{K}_B|Y^N_1=y^N_1, A \text{ selects } Y_1, A \text{ accepts } Y^N_1) \\
    &=\Pr(B \text{ selects } Y_1 | Y^N_1=y^N_1, A \text{ selects } Y_1, A \text{ accepts } Y^N_1) \\
    &= \Pr(B \text{ selects } Y_1 | Y^N_1=y^N_1, A \text{ selects } Y_1) \label{independent_to_explain} \\
    &\geq \left({1 + \frac{P^A_Y(y_1)}{P^B_Y(y_1)}\frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)}}\right) \quad \text{ (Importance Matching Lemma \cite{phan2024importance})} ,
\end{align}
where (\ref{independent_to_explain}) is due to the fact that conditioning on $Y^N_1=y^N_1, A \text{ selects } Y_1$ the event $\{B \text{ selects } Y_1\} $ is independent of the event $\{A \text{ accepts } Y^N_1\}$ by construction.

Furthermore, note that the event:
\begin{align}
    P(\Tilde{Y}^N_2=y^N_2| Y_{K_A}=y_1, K_{2,A} = 1) &= \frac{\Bar{P}_{Y,{K_{2,A}}}(y^N_1, 1)}{P^A_Y(y_1)N^{-1}}\\
    &= \frac{N Q_Y(y^N_2)}{\Delta_{P^A_Y} (\hat{Z}(P^A_Y, y^N_2) + \omega)}
\end{align}
where $\Bar{P}_{Y,{K_{2,A}}}(y^N_1, 1)$ is the ERS target distribution (\ref{ERS_target_distribution}) and $\Delta_{P^A_Y} < 1$ is the normalized constant.
Combining the two expressions, we have:
\begin{align}
    &\Pr(Y_{K_A} = Y_{\Tilde{K}_B}| Y_{K_A} = y)\\ &\geq \mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{N}{(\hat{Z}(P^A_Y, y^N_2) + \omega) \Delta_{P^A_Y} \left( 1 + \frac{P^A_Y(y_1)}{P^B_Y(y1)}\frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)}\right)}\right] \\
    &\geq \mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{N}{(\hat{Z}(P^A_Y, y^N_2) + \omega)  \left( 1 + \frac{P^A_Y(y_1)}{P^B_Y(y1)}\frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)}\right)}\right] \quad \text{(Since } \Delta_{P^A_Y} \leq 1)\\
    &\geq \left(\mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{(\hat{Z}(P^A_Y, y^N_2) + \omega)}{N} \left( 1 + \frac{P^A_Y(y_1)}{P^B_Y(y1)}\frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)}\right)\right]\right)^{-1} (\text{ By Jensen's Inequality} ) \label{left_off}
\end{align}

We then have:
\begin{align}
    \mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{\hat{Z}(P^A_Y, y^N_2) + \omega}{N}\right] &\leq \frac{N-1}{N} + \frac{\omega}{N}  \label{left_off1}
\end{align}
and:
\begin{align}
     &\mathbb{E}_{Y^N_2 \sim Q_Y}\left[\left(\frac{\hat{Z}(P^A_Y, y^N_2) + \omega}{N}\right)\frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)}\right]\\
     &= \mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{\hat{Z}(P^A_Y, y^N_2)}{N}\frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)} + \frac{\omega}{N} \frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)}\right] \\
     &\leq \frac{N-1}{N} + \frac{P^B_Y(y_1)/Q_Y(y_1)}{N} + \frac{\omega}{N}\mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)}\right]  \label{left_off2}
\end{align}

where we have:
\begin{align}
    \mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{\hat{Z}(P^B_Y, y^N_1)}{\hat{Z}(P^A_Y, y^N_1)}\right] &= \mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{P^B_Y(y_1)/Q_Y(y_1)}{\hat{Z}(P^A_Y, y^N_1)} + \frac{\hat{Z}(P^B_Y, y^N_2)}{\hat{Z}(P^A_Y, y^N_1)}\right] \\
    &\leq \mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{P^B_Y(y_1)/Q_Y(y_1)}{P^A_Y(y_1)/Q_Y(y_1)}\right] + \mathbb{E}_{Y^N_2 \sim Q_Y}\left[\frac{\hat{Z}(P^B_Y, y^N_2)}{\hat{Z}(P^A_Y, y^N_2)}\right]  \\
    &\leq \frac{P^B_Y(y_1)}{P^A_Y(y_1)} + \mathbbm{I}_N(\omega,2)d_2(Q_Y||P^A_Y)  \label{left_off3}
\end{align}

Then, combining (\ref{left_off3}) into (\ref{left_off2}), then combine with (\ref{left_off1}) into the term (\ref{left_off}), we have:
\begin{align}
    &\Pr(Y_{K_A} = Y_{\Tilde{K}_B}| Y_{K_A} = y)\\
    &\geq \left(1 + \frac{\omega}{N} + \frac{P^A_Y(y_1)}{P^B_Y(y_1)} \left(\frac{N-1}{N} + \frac{P^B_Y(y_1)/Q_Y(y_1)}{N} + \frac{\omega}{N} \left(\frac{P^B_Y(y_1)}{P^A_Y(y_1)} + \mathbbm{I}_N(\omega,2)d_2(Q_Y||P^A_Y)\right)\right)\right)^{-1}\\
    &= \left(1 + \frac{\omega}{N} + \frac{P^A_Y(y_1)}{P^B_Y(y_1)} \left(\frac{N-1}{N} + \frac{P^B_Y(y_1)/Q_Y(y_1)}{N} + \frac{\omega}{N} \left(\frac{P^B_Y(y_1)}{P^A_Y(y_1)} + \mathbbm{I}_N(\omega,2)d_2(Q_Y||P^A_Y)\right)\right)\right)^{-1} \\
    &\geq \left(1 + \frac{3\omega}{N} + \frac{P^A_Y(y_1)}{P^B_Y(y_1)} \left(1 +  \frac{\omega}{N} \mathbbm{I}_N(\omega,2)d_2(Q_Y||P^A_Y)\right)\right)^{-1} \\
    &= \left(1 + \mu'_1(N) + \frac{P^A_Y(y_1)}{P^B_Y(y_1)} \left(1 +  \mu'_2(N)\right)\right)^{-1},
\end{align}
where we repeatly use the fact that $P^A_Y(y)/Q_Y(y) \leq \omega$. This completes the proof.



==> protocol.tex <==

\begin{algorithm}[H]
\centering
\caption{Wyner-Ziv Distributed Compression Protocol}
\label{comm_protocol}

\begin{minipage}{\linewidth}
\textbf{Encoder:} Receives $X = x$ and $W$, performs:
\vspace{-5pt}
\begin{flalign*}
&\text{1. Select } K_A = \mathrm{ERS}(W; P_{Y'|X=x}, Q_{Y'}); \quad 
\text{2. Sends } (K_{1,A}, V_{K_A}) \text{ to the decoder.} &&
\end{flalign*}

\vspace*{-5pt}
\textbf{Decoder:} Receives $Z = (V_{K_A}, K_{1,A}, X')$ and $W$, performs:
\vspace{-5pt}
\begin{flalign*}
&\text{1. Keep batch } K_{1,A}; \quad 
\text{2. Remove all $j$ where } V_{K_{1,A},j} \neq V_{K_A}; \quad 
\text{3. Select } K_B \text{ with } P_{Y'|X'=x'}. &&
\end{flalign*}
\end{minipage}
\end{algorithm}

==> tables/Gaussian_table.tex <==
\begin{figure}[t]
\begin{minipage}{0.3\linewidth}
  \centering
\resizebox{\textwidth}{!}{\begin{tabular}{@{}p{1.8cm}p{3.5cm}@{}}
\toprule
\textbf{Distribution} & \textbf{Expression} \\
\midrule
\(Q_{Y'}(\cdot)\) & \(\mathcal{N}(0, \sigma^2_{Y'})\) \\ \addlinespace[2pt]
\(P_{Y'|X}(\cdot\,|\,x)\) & \(\mathcal{N}(x, \sigma^2_{Y'|X})\) \\
\(P_{Y'|X'}(\cdot\,|\,x')\) & \(\mathcal{N}\left(x' \frac{\sigma^2_X}{\sigma^2_{X'}}, \, \sigma^2_{Y'} - \frac{\sigma^4_X}{\sigma^2_{X'}}\right)\) \\
\bottomrule
\end{tabular}\hspace*{-0.5mm}}
\end{minipage}
\begin{minipage}{0.25\linewidth}
  \centering
\resizebox{\textwidth}{!}{\begin{tabular}{@{}p{1.8cm}p{3.5cm}@{}}
\toprule
\textbf{Distribution} & \textbf{Expression} \\
\midrule
\(Q_{Y'}(\cdot)\) & \(\mathcal{N}(0, \sigma^2_{Y'})\) \\ \addlinespace[2pt]
\(P_{Y'|X}(\cdot\,|\,x)\) & \(\mathcal{N}(x, \sigma^2_{Y'|X})\) \\
\(P_{Y'|X'}(\cdot\,|\,x')\) & \(\mathcal{N}\left(x' \frac{\sigma^2_X}{\sigma^2_{X'}}, \, \sigma^2_{Y'} - \frac{\sigma^4_X}{\sigma^2_{X'}}\right)\) \\
\bottomrule
\end{tabular}\hspace*{-0.5mm}}
\end{minipage}
\begin{minipage}{0.6\linewidth}
  \centering
\end{minipage}
\vspace*{-3mm}
\caption{Pass rates for the HumanEval Random Span benchmark
  from \citet{bavarian2022efficient} with {\tt CodeLlama-7b}
  for infilling Python.
  Across all settings, the byte-level predictions yield better completions.
  We evaluate the two standard infilling prompt templates of {\tt Prefix-Suffix-Middle} (PSM)
  and {\tt Suffix-Prefix-Middle} (SPM), and as baselines use token healing \citep{dagan2024getting} and alignment \citep{athiwaratkun2024token}.
  The SPM template forces the model to make predictions from the middle of a token,
  which our byte-level predictions successfully handle. 
}
\label{fig:fim}
\vspace{-15pt}
\end{figure}
